Cloud-based XAI Services for Assessing Open Repository Models Under Adversarial Attacks

The opacity of AI models necessitates both validation and evaluation before their integration into services. To investigate these models, explainable AI (XAI) employs methods that elucidate the relationship between input features and output predictions. The operations of XAI extend beyond the execution of a single algorithm, involving a series of activities that include preprocessing data, adjusting XAI to align with model parameters, invoking the model to generate predictions, and summarizing the XAI results. Adversarial attacks are well-known threats that aim to mislead AI models. The assessment complexity, especially for XAI, increases when open-source AI models are subject to adversarial attacks, due to various combinations. To automate the numerous entities and tasks involved in XAI-based assessments, we propose a cloud-based service framework that encapsulates computing components as microservices and organizes assessment tasks into pipelines. The current XAI tools are not inherently service-oriented. This framework also integrates open XAI tool libraries as part of the pipeline composition. We demonstrate the application of XAI services for assessing five quality attributes of AI models: (1) computational cost, (2) performance, (3) robustness, (4) explanation deviation, and (5) explanation resilience across computer vision and tabular cases. The service framework generates aggregated analysis that showcases the quality attributes for more than a hundred combination scenarios.

==> Sections/RQs.tex <==
\section{Research Questions}


\begin{algorithm}
\caption{Calculation of Explanation Metrics}
\label{eq:stability_metric}
\begin{algorithmic}[1]
\State \textbf{Input:} Set of explanation summaries \(E = \{\xi^{1}, \xi^{2}, \ldots, \xi^{m}\}\)
\State \textbf{Output:} \(f_d^{K}\) (Stability); \(f_d^{X}\) (Consistency)

\Statex \textit{Notations:}
\Statex \( m \) - Number of summaries in \(E\)
\Statex \( K \) - Combinations, \( \binom{m}{2} \)
\Statex \( \xi^{i} \) - \(i\)-th explanation summary
\Statex \( \xi^{X} \) - Summary for XAI method \(X\)
\Statex \( f_d^{[k]} \) - Prediction changes for \(k\)-th pair

\Procedure{Explanation Stability}{E}
    \State \( K \gets \binom{m}{2} \)
    \State \( f_d^{K} \gets \frac{1}{K} \sum_{k=1}^{K} f_d^{[k]}(\xi^{i},\xi^{j}) \) where \(i \neq j\), \(i,j \leq m\)
\EndProcedure

\Procedure{Explanation Consistency}{E, X}
    \State \( f_d^{X} \gets \frac{1}{m-1} \sum_{k=1}^{m-1} f_d^{[k]}(\xi^{X},\xi^{i}) \) where \(i \leq m\)
\EndProcedure

\end{algorithmic}
\end{algorithm}

\subsection{Consistency, Stability, and Generality of Explanations}
\begin{itemize}
    \item RQ1: Do CAM-based XAI methods offer consistent and stable explanations across different AI models such as the ViT, CVT, and Swin Transformer?
    \item RQ2: How does the stability of explanations change with different input perturbations, such as those from ImageNet-C (e.g., noise, blur)?
    \item RQ3: Can our XAI service framework easily adapt and explain other models on Hugging Face?
    \item RQ4: Is our framework still effective for AI models not hosted on Hugging Face?
\end{itemize}

\subsection{Computational Resource Assessment}
\begin{itemize}
    \item RQ5: What is the computational cost of providing explanations for AI models? Is there a significant variance depending on the model or XAI method used?
    \item RQ6: How much computational overhead does the XAI service framework add compared to traditional model evaluation?
\end{itemize}

\subsection{Resilience Against Adversarial Attacks}
\begin{itemize}
    \item RQ7: Can our XAI framework provide meaningful explanations when subjected to adversarial attacks?
    \item RQ8: Is there a correlation between the robustness of the model and the consistency of its explanations under adversarial attacks?
\end{itemize}

\subsection{Observations on XAI Outcomes Under Adversarial Attacks}
\begin{itemize}
    \item RQ9: Given adversarial attacks, how do the XAI outcomes change? 
    \item RQ10: What distinct observations and insights can be drawn from the XAI results under these adversarial conditions?
\end{itemize}

\subsection{Scientific Innovations and Contributions}
\begin{itemize}
    \item RQ11: How does our XAI framework pioneer the direct interpretation and evaluation of models from open-source repositories like Hugging Face, filling the existing gap in the community?
    \item RQ12: What novel methodologies or techniques does our framework introduce to enhance the explainability and evaluability of open-source AI models?
    \item RQ13: To what extent does our framework standardize and streamline the process of obtaining explanations for a wide range of open-source models, promoting reproducibility and transparency in the AI community?
    \item RQ14: How does our framework's capability to adapt and provide end-to-end explanations for diverse models reshape the landscape of model interpretability in open-source platforms?
    \item RQ15: How do CAM-based XAI methods compare in terms of consistency and stability across different AI models, such as the ViT, CVT, and Swin Transformer?
\item RQ16: What is the impact of different input perturbations, such as noise and blur from ImageNet-C, on the stability of explanations provided by CAM-based XAI methods?
\end{itemize}


\section{Equations}


\subsection*{PCD}
PCD
Let:
\begin{itemize}
    \item \( S_{\text{original}} \): Score of the top-1 class for the original image.
    \item \( S_{\text{masked}} \): Score of the top-1 class for the masked image.
\end{itemize}

Then, the change in prediction is defined as:
\[ \Delta_{\text{change}} = \left| S_{\text{original}} - S_{\text{masked}} \right| \]

And the percentage change relative to the original score is:
\[ \text{Percentage}_{\text{change}} = \frac{\Delta_{\text{change}}}{\left| S_{\text{original}} \right|} \]

KL
Let:
\begin{itemize}
    \item \( P_{\text{original}}(i) \): Softmax probability of the \(i\)-th class for the original image.
    \item \( P_{\text{masked}}(i) \): Softmax probability of the \(i\)-th class for the masked image.
\end{itemize}

Convert the logits to softmax probabilities:
\begin{align*}
P_{\text{original}}(i) &= \frac{\exp(\text{logits}_{\text{original}}(i))}{\sum_{j}\exp(\text{logits}_{\text{original}}(j))} \\
P_{\text{masked}}(i) &= \frac{\exp(\text{logits}_{\text{masked}}(i))}{\sum_{j}\exp(\text{logits}_{\text{masked}}(j))}
\end{align*}

Compute the KL Divergence:
\[ D_{KL}(P_{\text{original}}||P_{\text{masked}}) = \sum_{i} P_{\text{original}}(i) \log \frac{P_{\text{original}}(i)}{P_{\text{masked}}(i)} \]

Normalize the KL Divergence:
\[ \text{Normalized } D_{KL} = \frac{D_{KL}(P_{\text{original}}||P_{\text{masked}})}{\log(\text{len}(P_{\text{original}}))} \]





\section*{Extra Overhead Analysis Due to XAI in MLOps}

For analyzing the extra overhead introduced by XAI in MLOps, we can consider both time and energy overheads. 

\begin{equation}
R_{\text{time}} = \frac{T_{\text{XAI}}}{T_{\text{ML}} + T_{\text{XAI}}} \times 100\%
\end{equation}

Where:
\begin{itemize}
    \item \( R_{\text{time}} \) is the percentage of time overhead due to XAI.
    \item \( T_{\text{XAI}} \) is the time taken by the XAI method.
    \item \( T_{\text{ML}} \) is the time taken by the ML method without XAI.
\end{itemize}

\begin{equation}
R_{\text{energy}} = \frac{E_{\text{XAI}}}{E_{\text{ML}} + E_{\text{XAI}}} \times 100\%
\end{equation}

Where:
\begin{itemize}
    \item \( R_{\text{energy}} \) is the percentage of energy overhead due to XAI.
    \item \( E_{\text{XAI}} \) is the energy consumed by the XAI method.
    \item \( E_{\text{ML}} \) is the energy consumed by the ML method without XAI.
\end{itemize}


\section*{Mean Absolute Error (MAE)}

The Mean Absolute Error (MAE) is defined as:
\[
MAE = \frac{1}{n} \sum_{i=1}^{n} |y_i - \hat{y}_i|
\]

Where:
\begin{itemize}
    \item \( n \) is the total number of data points.
    \item \( y_i \) is the actual value of the i-th observation.
    \item \( \hat{y}_i \) is the predicted value of the i-th observation.
\end{itemize}

\subsection*{Comparison using MAE}

1. Image with and without Adversarial perturbation:
\[
MAE_{\text{image}} = \frac{1}{n} \sum_{i=1}^{n} |y_{\text{image, true}, i} - \hat{y}_{\text{image, perturbed}, i}|
\]

2. XAI with and without Adversarial perturbation:
\[
MAE_{\text{XAI}} = \frac{1}{n} \sum_{i=1}^{n} |y_{\text{XAI, true}, i} - \hat{y}_{\text{XAI, perturbed}, i}|
\]

\subsection*{Comparison using SSIM}
Given two windows \( x \) and \( y \) from two images, the Structural Similarity Index (SSIM) between them is defined as:

\begin{equation}
\text{SSIM}(x, y) = \frac{(2\mu_x\mu_y + C_1)(2\sigma_{xy} + C_2)}{(\mu_x^2 + \mu_y^2 + C_1)(\sigma_x^2 + \sigma_y^2 + C_2)}
\end{equation}

Where:
\begin{itemize}
\item \( \mu_x \) and \( \mu_y \) are the means of windows \( x \) and \( y \) respectively.
\item \( \sigma_x^2 \) and \( \sigma_y^2 \) are the variances of windows \( x \) and \( y \) respectively.
\item \( \sigma_{xy} \) is the covariance between windows \( x \) and \( y \).
\item \( C_1 \) and \( C_2 \) are small constants added for stability.
\end{itemize}



The Structural Similarity Index (SSIM) for comparing two images, \( x \) and \( y \), is defined as:
\[
SSIM(x, y) = \frac{(2\mu_x \mu_y + c_1)(2\sigma_{xy} + c_2)}{(\mu_x^2 + \mu_y^2 + c_1)(\sigma_x^2 + \sigma_y^2 + c_2)}
\]

Where:
\begin{itemize}
    \item \( \mu_x \) and \( \mu_y \) are the average of \( x \) and \( y \) respectively.
    \item \( \sigma_x^2 \) and \( \sigma_y^2 \) are the variances of \( x \) and \( y \) respectively.
    \item \( \sigma_{xy} \) is the covariance of \( x \) and \( y \).
    \item \( c_1 \) and \( c_2 \) are constants to avoid division by zero.
\end{itemize}


Given two images \(I_1\) and \(I_2\), the Mean Absolute Error (MAE) between them is defined as:

\begin{equation}
\text{MAE}(I_1, I_2) = \frac{1}{N} \sum_{i=1}^{N} |I_1(i) - I_2(i)|
\end{equation}

where \(N\) is the total number of pixels in the images.




\subsection*{Comparison using SSIM}

1. Image with and without Adversarial perturbation:
\[
SSIM_{\text{image}}(y_{\text{image, true}}, \hat{y}_{\text{image, perturbed}})
\]

2. XAI with and without Adversarial perturbation:
\[
SSIM_{\text{XAI}}(y_{\text{XAI, true}}, \hat{y}_{\text{XAI, perturbed}})
\]


\begin{algorithm}
\caption{Calculate Prediction Difference}
\begin{algorithmic}[1]
\Require Two sets of images: Original $O$ and Masked $M$
\Require Model $\mathcal{M}$ for prediction

\For{each image pair $o_i \in O$ and $m_i \in M$}
    \State Compute prediction score: $s_{o_i} \gets \mathcal{M}(o_i)$ and $s_{m_i} \gets \mathcal{M}(m_i)$
    \State Compute the difference: $d_i \gets |s_{o_i} - s_{m_i}|$
\EndFor

\State Compute the average difference:
\[
\bar{d} \gets \frac{1}{N} \sum_{i=1}^{N} d_i
\]
\State \Return $\bar{d}$

\end{algorithmic}
\end{algorithm}



\begin{table}[h!]
\centering
\caption{Performance of VIT Model under Different Adversarial Perturbation}
\label{table:performance_vit}
\begin{tabularx}{\linewidth}{lxxx}
\toprule
\textbf{Perturbation} & \textbf{Precision} & \textbf{Recall} & \textbf{F1 Score} \\
\midrule
Original & 0.7432 & 0.7432 & 0.7432 \\
\midrule
Gaussian Noise1 & 0.7003 & 0.7003 & 0.7003 \\
Gaussian Noise2 & 0.6853 & 0.6268 & 0.627 \\
Gaussian Noise3 & 0.5879 & 0.471 & 0.4789 \\
\midrule
Defocus Blur1 & 0.6689 & 0.6656 & 0.6677 \\
Defocus Blur2 & 0.6649 & 0.616 & 0.6135 \\
Defocus Blur3 & 0.5956 & 0.5065 & 0.5085 \\
\midrule
Pixelate 1 & 0.7652 & 0.7424 & 0.7416 \\
Pixelate 2 & 0.7617 & 0.7385 & 0.7377 \\
Pixelate 3 & 0.7318 & 0.7016 & 0.7003 \\
\bottomrule
\end{tabularx}
\end{table}


\begin{algorithm}
\caption{Calculation of Explanation Metrics \cite{xaiprocess}}
\label{eq:stability_metric}
\begin{algorithmic}[1]
\State \textbf{Input:} Set of explanation summaries \(E = \{\xi^{1}, \xi^{2}, \ldots, \xi^{m}\}\)
\State \textbf{Output:} \(f_d^{K}\) (Stability); \(f_d^{X}\) (Consistency)

\Statex \textit{Notations:}
\Statex \( m \) - Number of summaries in \(E\)
\Statex \( K \) - Combinations, \( \binom{m}{2} \)
\Statex \( \xi^{i} \) - \(i\)-th explanation summary
\Statex \( \xi^{X} \) - Summary for XAI method \(X\)
\Statex \( f_d^{[k]} \) - Prediction changes for \(k\)-th pair

\Procedure{Explanation Stability}{E}
    \State \( K \gets \binom{m}{2} \)
    \State \( f_d^{K} \gets \frac{1}{K} \sum_{k=1}^{K} f_d^{[k]}(\xi^{i},\xi^{j}) \) where \(i \neq j\), \(i,j \leq m\)
\EndProcedure

\Procedure{Explanation Consistency}{E, X}
    \State \( f_d^{X} \gets \frac{1}{m-1} \sum_{k=1}^{m-1} f_d^{[k]}(\xi^{X},\xi^{i}) \) where \(i \leq m\)
\EndProcedure

\end{algorithmic}
\end{algorithm}

==> Sections/architecture.tex <==
\section{Overview of XAI Assessment Quality Attribution}
\label{chap:architecture}

% The guide \cite{lones2021avoid} suggests researchers evaluate models and compare models to avoid pitfalls.

\subsection{Service Components and Their Interactions}

The architecture pattern presented in Figure \ref{fig:servicearchitecture} outlines a structured approach to delivering XAI services within a cloud environment. This service-oriented architecture is designed to facilitate the analysis and comparison of various AI models through a suite of microservices, each dedicated to a specific aspect of XAI evaluation. The main components of this architecture include:

\paragraph{Open APIs} The interface allows users to operate the XAI process. This interface is designed to be accessible by software, ensuring that users can easily interact with the XAI.

\paragraph{Integrated SDKs} Parallel to the Open APIs, SDKs provide a programmatic way to execute service tasks. It's convenient for developers and researchers who operate the process or integrate it into their existing workflows programmatically.

\paragraph{Coordination Center} A microservice that executes the XAI pipeline. It communicates with other microservices according to tasks, records provenance data for transparency and reproducibility. 

\paragraph{Data Processing Service} The microservice is responsible for transforming and preprocessing data. It ensures that data is formatted correctly and aligned with the requirements of the XAI algorithm. Also, it can apply adversarial perturbations \cite{imagenetC} to the dataset for testing robustness.

\paragraph{AI Model Service} This encapsulates the pre-trained AI models within the service framework. The AI models, including the open-sources model from the HuggingFace Community, can be encapsulated and deployed. The designed API rules ensure integration with the coordination center.

\paragraph{XAI Method Service} This service offers XAI that can generate explanations. XAI algorithms \cite{Trustworthy} and tool libraries  \cite{yang2022omnixai} can be encapsulated into the service. 
The service can execute XAI computing with the corresponding microservices.

\paragraph{Evaluation Service} This service aggregates the results and conducts systematic evaluations of the defined quality attributes, thereby ensuring the quality of AI systems.

Together, these components form the cloud-based architecture that supports the end-to-end model evaluation process with XAI and adversarial perturbations. 



